Residual Parameter Transfer for Deep Domain Adaptation

The goal of Deep Domain Adaptation is to make it possible to use Deep Nets trained in one domain where there is enough annotated training data in another where there is little or none. Most current approaches have focused on learning feature representations that are invariant to the changes that occur when going from one domain to the other, which means using the same network parameters in both domains. While some recent algorithms explicitly model the changes by adapting the network parameters, they either severely restrict the possible domain changes, or significantly increase the number of model parameters. By contrast, we introduce a network architecture that includes auxiliary residual networks, which we train to predict the parameters in the domain with little annotated data from those in the other one. This architecture enables us to flexibly preserve the similarities between domains where they exist and model the differences when necessary. We demonstrate that our approach yields higher accuracy than state-of-the-art methods without undue complexity.

==> analysis.tex <==
%% -*- mode: latex; mode: reftex; mode: flyspell; TeX-master: "top; -*-

\section{Automatic architecture selection}

As we can see from \eqt{deep_weights} our method depends on the choice of the rank of the transformation that is relating the weights of different streams. As we show in our experiments setting rank arbitrary allows to significantly improve performance, comparing to the approach of~\cite{Ganin15}, which essentially has the same architecture as us, but the weights between streams are shared. However, achieving the optimal performance required careful selection of rank $k$, which may be different for all the layers.

This, on the other hand, may be time consuming for relatively large networks (such as VGG~\cite{Simonyan15} or GoogleNet~\cite{Szegedy15}), as in order to find the optimal configuration we would need to run our approach several times and then use, e.g. Maximum Mean Discrepancy criterion, suggested by~\cite{Rozantsev16b}. Inspired by~\cite{Alvarez16a} we would like to avoid this by automatically learning the transformation rank $k$ for all the layers of the two-stream architecture. 

We suggest using sparse group Lasso idea, which was originally proposed by~\cite{Simon13}. Therefore, we propose to add a similar regularizer as~\cite{Alvarez16a}, however applied not to the neurons, but to the rows of matrices $\bbeta$:
%
\begin{equation}
r(\bbeta) = \lambda_l \sum_{i \in \Omega} \left( (1-\gamma)\sqrt{N_i}\sum_{j = 1}^{k_i} \norm{\beta_i^j}_2 + \gamma \norm{\beta_i}_1 \right)
\label{eq:group_lasso_reg}
\end{equation}
\noindent
with $\gamma$ being the parameter that allows balancing between group sparsity term and the $L_1$ norm applied to the parameters $\bbeta$. We would then like to find such $\bbeta$ that both \eqt{cost_function} and \eqt{group_lasso_reg} are minimized.
This can be achieved by solving the following optimization problem 
%
\begin{equation}
\bbeta = \arg\min_{\bbeta} \frac{1}{2t}\norm{\bbeta - \hat{\bbeta}}_2^2 + r(\bbeta),
\label{eq:group_lasso_opt}
\end{equation}
\noindent
where $\hat{\bbeta} = \{\hat{\beta_i}\}_{i \in \Omega}$ is the solution obtained from minimizing \eqt{cost_function}. As shown by~\cite{Alvarez16a}, we can then solve \eqt{group_lasso_opt} in the closed-form for each $\beta_i$
%
\begin{equation}
\beta_i = \max{\left(0, 1 - \frac{t(1 - \gamma)\lambda_l\sqrt{N_i}}{\norm{S(\hat{\beta_i},t\gamma\lambda_l)}_2}\right)}S(\hat{\beta_i},t\gamma\lambda_l),
\label{eq:close_form_solution}
\end{equation}
\noindent
with $(S(z,\tau))_j = sign(z_j)\max{\left(0, |z_j|-\tau\right)}$.

This will force some of the rows in matrices $\bbeta$ go to zero, which essentially means that will no longer be used in optimization. This allows reducing the transformation rank $k_i$ between for some of the pairs of layers in the two-stream architecture. Further the fact that corresponding layers share their parameters will simply mean that the transformation rank $k_i$ for this pair is equal to zero.

The optimization then proceeds by taking a predefined number of gradient steps based on the loss function defined in \eqt{cost_function} and then updating the $\bbeta$ parameters according to \eqt{group_lasso_opt}. 

\section{Implementation details}

As the formulated optimization problem is quite complex, in this section we discuss different issue that we have faced during the network training and how they can be overcome.

\subsection{Optimization strategies}

Modern deep learning libraries do not support dynamically changing the network architecture. In our case, however, by allowing the transformation rank to be $0$ we allow the network architecture to change from non-shared weights in some of the layers to sharing them.


